Strictly Low Rank Constraint Optimization -- An Asymptotically $\mathcal{O}(\frac{1}{t^2})$ Method

We study a class of non-convex and non-smooth problems with \textit{rank} regularization to promote sparsity in optimal solution. We propose to apply the proximal gradient descent method to solve the problem and accelerate the process with a novel support set projection operation on the singular values of the intermediate update. We show that our algorithms are able to achieve a convergence rate of $O(\frac{1}{t^2})$, which is exactly same as Nesterov's optimal convergence rate for first-order methods on smooth and convex problems. Strict sparsity can be expected and the support set of singular values during each update is monotonically shrinking, which to our best knowledge, is novel in momentum-based algorithms.

==> preliminaries.tex <==
\section{Preliminaries}\label{sec:pre}

\subsection{Notations}
Throughout this paper, we use uppercase bold letters for matrices, lowercase bold letters for vectors, and lowercase letters for scalars. We use superscript to represent the current iteration. $\sigma_i (\cdot)$ is  the $i-$th largest singular value of a matrix, $\sigma_{min} (\cdot)$ and $\sigma_{max} (\cdot)$ represent the smallest and the largest singular value of a matrix, respectively, $\sigma(\cdot)$ indicates the vector formed by the singular values of a matrix, and $\dg(\sigma(\cdot))$ denotes the diagonal matrix formed by the vector. $|\cdot|$ denotes the cardinality of a set, supp$(\cdot)$ denotes the support of a vector. For a matrix $\xm \in \mathbb{R}^{n \times k}$, let $\sigma(\xm) = (\sigma_{max} (\xm), \sigma_2 (\xm), \dots, \sigma_{min} (\xm))$, then we can see rank$(\xm) = \|\sigma(\xm)\|_0$. 
$S = \sp(\sigma(\xm^0))$, $\xm^0$ is the initialization. 
The proximal mapping associated with $h(\cdot)$ is defined as $\textrm{prox}_h(\um) = \argmin_{\vm} h(\vm) + \frac{1}{2} \|\um-\vm\|^2_F$. 



\subsection{Assumptions}
In this paper, 
$g(\xm)$ in Eq.~(\ref{eq:fx}) is assumed to satisfy the following assumptions:
\begin{assumption}
1) g($\cdot)$ is convex, and $\nabla g(\cdot)$ has bounded singular value $\sigma_{max}(\nabla g(\xm))) \leq G$ for any $\xm$;

2) g($\cdot)$ has L-Lipschitz continuous gradient, $\| \nabla g(\xm_1) - \nabla g (\xm_2) \|_F \leq L\|\xm_1 - \xm_2\|_F$.
\label{ass:gx}
\end{assumption}

For the choice of $g(\cdot)$ in this paper, we let it be the squared loss $\|\ym - \dm \xm\|_F^2$, where $\ym \in \mathbb{R}^{d \times k}, \dm \in \mathbb{R}^{d \times n},\xm \in \mathbb{R}^{n \times k}$. 
